Accelerating Large Language Models through Partially Linear Feed-Forward Network

Large language models (LLMs) demonstrate remarkable capabilities but face deployment challenges due to their massive parameter counts. While existing compression techniques like pruning can reduce model size, it leads to significant accuracy degradation under high compression ratios. We present a novel perspective inspired by constant folding in compiler optimization. Our approach enables parameter reduction by treating activation functions in LLMs as linear functions. However, recent LLMs use complex non-linear activations like GELU that prevent direct application of this technique. We propose TARDIS, which enables optimization of LLMs with non-linear activations by partially approximating them with linear functions in frequently occurring input ranges. For outlier inputs, TARDIS employs an online predictor to dynamically fall back to original computations. Our experiments demonstrate that TARDIS achieves 80% parameter reduction in feed-forward networks, while significantly outperforming state-of-the-art pruning methods Wanda and RIA with up to 65% higher accuracy. In practical deployments for a 7B model, TARDIS achieves 1.6x end-to-end inference speedup when integrated with the vLLM serving system, and 1.4x speedup with the widely adopted HuggingFace implementation, while incurring only a 10.9% accuracy trade-off.

==> Makefile <==
#DOC_NAME    := castm
DOC_NAME    := paper

PS2PDF      := ps2pdf14

#use the following options to avoid the embedded font problem.
DVIPS       := dvips -j0 -Ppdf -Pdownload35 -G0 -t letter -D 1200 -Z -mode ljfzzz
LATEX       := pdflatex
FIG2DEV     := fig2dev

#use the following options to generate into a single html.
LATEX2HTML  := latex2html -split 0 -split +0 -link 0 -no_navigation -no_footnode -show_section_numbers -local_icons
DOXYGEN     := doxygen
BIBTEX	    := bibtex

BASE := Makefile $(wildcard *.tex) $(wildcard *.bib)
BASE := $(BASE) $(wildcard ./pic/*.eps)

PSOPT 	:=  -dNOPAUSE -dBATCH \
	-sDEVICE=pdfwrite -dPDFSETTINGS=/prepress\
	-dCompatibilityLevel=1.5 \
	-dCompressPages=true -dUseFlateCompression=false \
	-sPAPERSIZE=letter \
	-dSubsetFonts=true -dEmbedAllFonts=true \
	-dProcessColorModel=/DeviceGray \
	-dDetectBlends=true -dOptimize=true \
	-dDownsampleColorImages=true -dColorImageResolution=1200 \
	-dColorImageDownsampleType=/Average -dColorImageFilter=/FlateEncode \
	-dAutoFilterColorImages=false -dAntiAliasColorImages=false \
	-dColorImageDownsampleThreshold=1.50000 \
	-dDownsampleGrayImages=true -dGrayImageResolution=1200 \
	-dGrayImageDownsampleType=/Average -dGrayImageFilter=/FlateEncode \
	-dAutoFilterGrayImages=false -dAntiAliasGrayImages=false \
	-dGrayImageDownsampleThreshold=1.50000 \
	-dDownsampleMonoImages=true -dMonoImageResolution=1200 \
	-dMonoImageDownsampleType=/Average -dMonoImageFilter=/FlateEncode \
	-dAutoFilterMonoImages=false -dAntiAliasMonoImages=false \
	-dMonoImageDownsampleThreshold=1.50000

all: pdf


pdf: $(DOC_NAME).pdf

%.pdf: %.ps
	$(PS2PDF) $(PSOPT) $< $@
	@cat $(DOC_NAME).log | grep Warning

%.ps: %.dvi
	$(DVIPS) $< -o $@

%.dvi: $(BASE)
	@make clean
	set -x
	# @cd figure; ./plot.sh
	# @cd figures; ./plot.sh
	# @cd figure-new; python3 plot.py
	@cd gnuplot/scripts; ./plot_all.sh
	$(LATEX) $*.tex
	$(BIBTEX) $*
	$(LATEX) $*.tex
	$(BIBTEX) $*
	$(LATEX) $*.tex

plot:
	@cd gnuplot/scripts; ./plot_all.sh

html: $(DOC_NAME)/$(DOC_NAME).html

%.html: $(BASE)
	@rm -rf $(DOC_NAME)
	$(LATEX2HTML) $*.tex

clean:
	@rm -rf *.pdf *.ps *.dvi *.aux *.log *.bbl  *.blg *.idx *.out *~ pic/*~ $(DOC_NAME)

.PHONY: clean all pdf html

### Makefile ends here


==> algo/v2/graph_generation_new.tex <==
\begin{algorithm}[t]
    \caption{Dependency graph construction.}
    % \caption{Dependency graph construction with \ce}
    \label{alg:graph-generation-new}

    \begin{footnotesize}
        \let\oldgets\gets
        \renewcommand{\gets}{\textrm{ := }}
        
        \tt
        \underline{ConstructDG(ExternalState state, Instruction[] instructions)}:\\
        vertex = nil; curConds = true; graph = emptyGraph; store = \{\}\\
        markSymbolic(state.inputs, store) \codecomment{// mark the input state as symbolic}\\
        \textbf{foreach} \emph{instr} \textbf{in} \emph{instructions}:\\
        % \ \ globalVarDetection(instr)\\
        % \ \ \ \ \ \ \emph{operand} = getRecordedInput(\emph{operand}, \emph{records})\\
        % \ \ \ \ if \emph{operand} is global or input:\\
        % \ \ \ \ \ \ markSymbolic(\emph{operand})\\
        \ \ \textbf{switch} \emph{instr}:\\
        \ \ \ \ \textbf{case} \emph{instr} \textbf{is} \emph{`invoke prepareQuery'}:\\
        \ \ \ \ \ \ vertex = createVertex(\emph{instr}.sql)\\
        \ \ \ \ \textbf{case} \emph{instr} \textbf{is} \emph{`invoke setParam'}:\\
        \ \ \ \ \ \ vertex.parameters.add(instr.idx, store[\emph{instr}.param])\\
        \ \ \ \ \textbf{case} \emph{instr} \textbf{is} \emph{`invoke execute'}:\\
        \ \ \ \ \ \ vertex.conditions = curConds\\
        \ \ \ \ \ \ queryRes = nextQueryResult(\emph{state.queryResults}) \\
        \ \ \ \ \ \ \codecomment{// continue execution with symbolic query result}\\
        \ \ \ \ \ \ markSymbolic(queryRes, store)\\
        \ \ \ \ \ \ vertex.queryResult = store[queryRes]\\
        \ \ \ \ \ \ \codecomment{// append the new vertex to the tail of the graph}\\
        \ \ \ \ \ \ graph.tail.children.add(vertex); graph.tail = vertex\\
        \ \ \codecomment{ // execute the instruction concolically}\\
        % \ \ \codecomment{ // update the path condition and symbolic store}\\
        \ \ ConcolicExecute(instr, curConds, store)\\
        \ \ \textbf{if} \emph{instr} \textbf{is} \emph{`external call'}:\\
        \ \ \ \ markSymbolic(nextReturnedValue(state.returnValues), store)\\
        \textbf{return} \emph{graph}\\
        \ \ \ \\
        \underline{ConcolicExecute(Instruction instr, PathCondition pc, SymbStore s)}:\\
        \textbf{if} \emph{instr} \textbf{is} \emph{`if e then s\_true else s\_false'}:\\
        \ \ \textbf{if} e == true: pc = pc $\land$ store[\emph{e}]; goto `s\_true';\\
        \ \ else\ \ \ \ \ \ \ \ \ \ pc = pc $\land$ $\neg$store[\emph{e}]; goto `s\_false';\\
        \textbf{if} \emph{instr} \textbf{is} \emph{`assign x=e'}: store[x] = e\\
        \textbf{if} \emph{instr} \textbf{is} \emph{`binOp x y to z'}:\\
        \ \ \codecomment{ // creating a binary symbolic expression, and updates the symbolic store}\\
        \ \ store[z] = binOpExp(store[x], store[y], instr.op)\\
        ...\\
        \ \ \\
        \underline{MergeGraph(Graph g, Graph t)}:\\
        \codecomment{// g: existing \dg, t: new graph constructed from another hot path} \\
        \texttt{equalVertices} = longestEqualVertexSequence(g, t) \\
        \textbf{foreach} \sn \textbf{in} t:\\
        \ \ \textbf{if} \sn \textbf{in} equalVertices:\\
        \ \ \ \ n = g.getEqualityVertex(\sn)\\
        \ \ \ \ n.conditions = n.conditions $\lor$ \sn.conditions\\
        \ \ \ \ \codecomment{// adjust the parent and child \sns for the merged \sn n accordingly}\\
        \ \ \ \ n.children.add(\sn.children)\\
        \textbf{return} g\\
        \let\gets\oldgets
    \end{footnotesize}
\end{algorithm}

==> sections/back.tex <==
\section{Problem Statement}
%-------------------------------------------------------------------------------
% 用一个paragraph
Constant folding is a compiler optimization technique that evaluates constant expressions at compile time. Such optimization leverages the associativity, commutativity and distributivity of different expressions to simplify program. Constant folding has remained a staple of compiler optimization for decades. Modern compilers widely implement this technique across various programming languages, including C~\cite{Optimize87:online}, Python~\cite{pythoncp39:online}, and SQL~\cite{SparkSQL40:online}. Recent years, deep learning (DL) workloads have also benefited from this optimization capability. 
For instance, in DL frameworks such as TensorFlow~\cite{TensorFl23:online}, ONNX Runtime~\cite{Graphopt58:online}, and PyTorch~\cite{TorchScr40:online}, \cf has all been integrated into the computation graph optimization process, improving the efficiency of various DL pipelines~\cite{TensorFl23:online,Develope9:online,TensorRT28:online,TensorFl6:online}.

% \begin{itemize}
%     \item The importance of constant folding
%     \begin{itemize}
%         \item has been a staple of compiler optimization for decades. It has been widely used in modern compilers, including 
%         \begin{itemize}
%             \item Programming Language (C++, Python, SQL)
%             \item Recent years, machine learning workloads have also enjoied the compilers' optimization capability. In ML compilers such as TensorFlow~\cite{TensorFl23:online}, ONNX Runtime and PyTorch, constant folding acts as an important optimization.
%         \end{itemize}
%         % \item The benefits of constant folding are two fold:
%         % \begin{itemize}
%         %     \item Reduce runtime computational cost. \GS{TODO: add example on DL workloads}
%         %     \item Reduce source code size. \GS{TODO: add example}
%         % \end{itemize}
%         % \item To investigate how constant folding can benefit real-world machine learning workloads, we examined 50 ML workflows from Kaggel \GS{TODO: or GitHub, HuggingFace}. We measured the performance of these workloads with and without the constant folding compiler optimization. We found that constant folding can be applied to xxx of the 50 workflows, and results in an average speedup of xxx $\times$. The most significant speedup reaches xxx $\times$.
%         % 广泛使用，而不是优化很重要
%     \end{itemize}
%     \item Why DL workflows can benefit from constant folding?
%     \begin{itemize}
%         \item The condition that constant folding works.
%         \item Why ML workflows match the conditions?
%     \end{itemize}
% \end{itemize}

\iffalse

\subsection{Large Language Models}
\begin{itemize}
    \item The basic building blocks of transformer-based LLM: Attention, MLP, Residual \GS{TODO: add figure}
    \item The overall workflow of LLM devides into two phases: \textit{prefill} and \textit{decode}.
    \begin{itemize}
        \item Prefill: generate the first token based on user prompt. Compute-intensive, takes xxx\% of inference time.
        \item Decode: generate the following tokens in an auto-aggressive manner. IO-intensive, tekes xxx\% of inference time.
    \end{itemize}
\end{itemize}
\subsection{LLM Inference on Edge Devices}
Deploying large language models on edge devices (e.g., mobile devices, personal computers) is benefical in several perspectives. 
First, on-device deployment eliminates the  network delays of sending data to the LLMs on the cloud. This reduces response time and benefits to many real-time applications, like chatbots, personal assistants, etc. 
Second, deploying LLMs on edge devices reduces the operational cost of the LLMs deploied on the cloud. This leads to a drop in the cost of serving LLMs for business usages.
Finally, on-device LLMs enhance user privacy by keeping the user's data locally.

\begin{itemize}
    \item Problem statement: However, the large memory requirement for LLMs makes the deployment on edge devices challenging. For instance, LLaMA-3 8B requires 8GB to store them in half-precision floating point format. While more than 88\% smartphones today have less than 8GB of RAM~\cite{movr}, far below the parameter storage requirement for a LLM inference workload.
    \item Existing lines of works that reduce LLM size: 
    \begin{itemize}
        \item Pruning
        \begin{itemize}
            \item Structured Pruning
            \item Unstructured pruning 
            \item Contexual pruning
        \end{itemize}
        \item Quantization
        \begin{itemize}
            \item Quantization aware training
            \item Post-training quantization
        \end{itemize}
        \item Knowledge distilation
        \item Low-rank decomposition
    \end{itemize}
\end{itemize}
\fi
% Constant Folding in LLMs:
% 一个paragraph
Recently, large language models is becoming an active topic in both literature and industary. 
Despite the widespread adoption of \cf in various deep learning workloads optimizations, little research has explored its potential application to LLMs. 
To understand this gap, we first analyze the key enabler for the application of \cf to DL workloads. Then, we
compare the workload characteristics of LLMs with deep learning, and shed some light on why LLMs lacks optimization opportunity for \cf.
% - in DL workloads, models structure are more various, for example the 

\textit{\textbf{Why \cf works in deep learning workloads?}} Constant folding only works well in conditions where the program have many expressions that evaluates to fixed values. In DL workloads, the variety of model structures and complexity in the pipeline design brings opportunity for \cf. 
% \begin{itemize}
%     \item The conditions that constant folding works
%     \item why DL workflow match?
% \end{itemize}
In one aspect, model structures in DL workflows are more diverse. For example, in natural language processing (NLP) tasks, models like LSTM~\cite{hochreiter1997long}, RNN~\cite{medsker2001recurrent}, BERT~\cite{BART83:online}, Electra~\cite{clark2020electra} etc., are widely used. In vision tasks, models like VGG~\cite{simonyan2015deepconvolutionalnetworkslargescale}, ResNet~\cite{he2015deepresiduallearningimage}, Inception~\cite{szegedy2016rethinking}, etc., are popular.
These models have different architectures, and the internal logics of these models are usually complex. For instance, in a LSTM model, the internal logics include the forget gate, input gate, output gate, etc. In vision models like VGG~\cite{simonyan2015deepconvolutionalnetworkslargescale}, the internal logics include the convolutional layers, pooling layers, fully connected layers, etc. The complexity of the internal logics in these models leaves more optimization opportunities, including \cf, for DL workflows. We examined xxx DL models from xxx, and found that \cf can be applied to xxx of the xx models, and results in an average speedup of xxx $\times$.
In contrast, large language models (LLMs) are mainly transformer-based models, which have a relatively simple architecture.
% One key advantage of LLMs is that they are general-purpose models, whereas deep learning models are usually tailored to specific tasks.
% Specifically, one single LLM (like GPT-4) is capable of text classification, translation, question answersing, etc. While in DL systems, realizing the above capabilities might require models with different architectures like LSTM, RNN and BERT.

In additional, the data preprocessing steps, including data cleaning and feature engineering, in DL workloads are more complicated than LLMs. DL workloads could require a large effort in data cleaning and feature engineering, whereas LLM workloads is relatively simpler: users just send prompt texts to the LLM, and wait for the generation of the response.
As a result, the variety of model structure and complexity in supplementary code (logics that are not directly related with model inference, e.g., data cleaning and feature engineering) leaves more optimization opportunities, including \cf, for DL workflows. For example, a user might declared a constant parameter inside the loop of a feature engineering procedure\GS{TODO: find example}. We examined xxx DL workflows from xxx, and found that \cf can be applied to xxx of the xx workflows.
% , and results in an average speedup of xxx $\times$.

\textit{\textbf{Why \cf does not work in LLMs?}}
Although the number of weights in LLMs are significantly larger than DL models, the internal building blocks and pipeline of LLM workloads are simpler.
Specifically, LLMs are usually a sequence of several transformer blocks.
\begin{figure}
    \caption{LLM architectures and linear/non-linear transformation illustration}
    \label{fig:transformers}
\end{figure}
As shown in \Cref{fig:transformers}, each transformer block mainly contains a Multi-head attention (MHA) module, followed by a MultiLayer-Perceptron (MLP) module. The residual connection and normalization further chains MHA and MLP into one transformer block. More concretely, a transformer block performs two kinds of transformation to its input: linear transformation and non-linear transformations. We notice that in essence, \cf is to \textit{replace a sequence of (constant) linear transformers with a constant value}. Consequently, only sequence of linear transformations in LLMs have a chance to get folded. However, the non-linear transformations (e.g., activation function, softmax, normalization) interleave with the linear transformations, leaving no opportunity for \cf. For instance, in \Cref{fig:transformers}, MLP performs three transformations: a linear ($X'=XW_1$), a non-linear ($X''=\sigma(X')$) and finaly another linear ($X''W_2$) transformation. Due to presence of the non-linear activation, the matrix multiplication of $XW_1$ and $W_2$ cannot be folded into $XW_1W_2$.

Apart from the simpler architecture, the pipeline of LLM workloads is also simpler. To use the LLM, users only write a few lines of code to initialize the tokenizer and model, then start to send prompt texts to the model (e.g., in HuggingFace Transformers~\cite{Transf37:online}, ollama~\cite{Ollama33:online} and vLLM~\cite{10.1145/3600006.3613165}). 
The simpler architecture and pipeline could leave little opportunity for \cf. We examined xxx LLM models from xxx, and found that \cf are not applicable to all of them.

% \begin{itemize}
%     \item Why \cf not work in llm?
%         \item llms are simpler
%         \item the simpler structure does not have \cf opportunity
%             \item llms are linear and non linear transformations
%             \item two consecutive linear transformation can be folded into one
%             \item due to the existence of "barrier" non-linear transformations, not able to fold
% \end{itemize}
% Formally, the MHA and MLP can be written as:
% $$
% \begin{align}
% Attention(Q,K,V)=Softmax(\frac{QK^T}{\sqrt{d}})V\\
% MultiHead(Q,K,V)=Concat(h_1,...,h_n)W^O\\
% where\ head_i=Attention(QW_i^Q,KW_i^K,VW_i^V)
% \end{align}
% $$
% $$
% MLP(x) = \sigma(xW_1)(W_2)
% $$
% $$
% \begin{align}
% Residual(f, X)=f(X)+X\\
% transformer_i(X)=Norm(MLP(
% Norm(Residual(MHA, X))))
% \end{align}
% $$
% \begin{itemize}
%     \item Comparison of DL workloads and LLM workloads
%     \begin{itemize}
%         \item The key difference between them: different from DL workloads that usually consists of different steps (i.e., data cleaning, feature engineering, model inference, etc.), LLM workloads is relatively simpler: users of LLM send prompt texts to the model, and wait for the generation of the response. Consequently, the core execution logic mainly lies in the internal of the model itself during response generation.
%         \item The internal of a LLM: transformer based model, which contains Multi-head attention and MLP.
%         \begin{itemize}
%             \item MHA
%             \item MLP:We start by a multilayer perceptron (MLP), which is the basic building block in the majority of large language models. Formally, a MLP consists of two weight matrixs $W_1\in\mathbb{R}^{d\times h}$ and $W_2\in\mathbb{R}^{h\times d}$, given an input $x\in\mathbb{R}^{n\times d}$, MLP is defined as follows:
%             $$
%             MLP(x) = \sigma(xW_1)(W_2)
%             $$
%             where $\sigma$ is an non-linear activation function (e.g., SiLU, GELU, etc.).
%         \end{itemize}
%     \end{itemize}
%     \item Why the internal of LLM is not \cf friendly?
%     \begin{itemize}
%         \item recap the condition of \cf
%         \item why LLM workload does not match the condition: ``barrier'' operations: non-linear operators, softmax, activation, layer-normalization
%     \end{itemize}
% \end{itemize}
\section{Strawman and challenge}
According to the above analysis, the primary barrier preventing LLMs achieving \cf lies in the non-linear transformations that interleave with linear transformations. To enable LLMs to be ``constant foldable'', we must adjust their structural design, allowing multiple linear transformations to chain together seamlessly.
\subsection{Strawman}
To enhance the \cf opportunities in LLMs, an intuitive idea would be modifying the non-linear transformations into linear ones. By removing these non-linear barriers, the resulting LLMs are more amenable to \cf.

% Consider the case of a MLP. We define a linear transformation function as follows:
Let us consider the case of modifying the non-linear activation function in MLP modules of an LLM. We define a linear transformation $\phi$ as follows:
\[
\phi(x) = ax + b
\]
where \(a, b\) are scaler values. We can approximate the original non-linear function \(\sigma\) in MLP with \(\phi\):
\[
\begin{aligned}
    MLP(x)=\sigma(xW_1)(W_2) \\
    \approx \phi(xW_1)(W_2) = (a(xW_1) + b)(W_2).
\end{aligned}
\]
where $W_1\in\mathbb{R}^{d\times h}$ and $W_2\in\mathbb{R}^{h\times d}$. This formulation effectively eliminates non-linear transformations, enabling us to constant folding the MLP into a simplified linear transformation:
\[
MLP(x) \approx \overline{MLP}(x) = (a(xW_1) + b)(W_2) = xC + B,
\]
where \(C \in \mathbb{R}^{d \times d}\) and \(B \in \mathbb{R}^{1 \times d}\). This transformation significantly alters the weight parameter count in the MLP, reducing it from \(2 \times d \times h\) to \(d^2 + d\) in \(\overline{MLP}\). Notably, when \(h > \frac{d + 1}{2}\), the number of weight parameters decreases after \cf.
In many contemporary LLMs employing this MLP block—such as OPT, BLOOM, and Falcon—\(h\) typically equals \(4d\). This configuration can yield a theoretical parameter reduction of up to 87.5\% (as \(d \rightarrow \infty\)) within the MLP blocks.

Apart from the MLP block, the MHA block can also be modified to increase \cf opportunities. 
However, the benefits of \cf in MHA are minimal, as the resulting folded matrices contains far more parameters than the original matrices. In this paper, we focus on \cf of MLP blocks in LLMs. These blocks takes up 67\%\ to 80\% of the total parameters in LLMs~\cite{almazrouei2023falconseriesopenlanguage,touvron2023llama2openfoundation}, and often takes up much computational and memory resources during inference~\cite{xu2024survey,zhou2024survey,lin2024awq,yuan2024llm}.

% Regarding multi-head attention (MHA), while we can achieve constant folding, the benefits are minimal. 

% The key challenge arises from non-linear operators, which hinder the constant folding process. By addressing these barriers, we can transform LLMs into structures that are amenable to constant folding.
% \begin{itemize}
%     \item To make LLMs constant foldable, an idea would be to modify the internal structure of LLM to increase \cf opportunities.
%     \item The barriers to \cf in LLMs are non-linear operators. If we modify the barriers, LLMs are constant foldable.
%     \item MLP: For example, Let us consider a function that performs linear transformation: $\phi(x)=ax+b$, where $a,b\in\mathbb{R}^{1\times h}$. We approximate the original non-linear function $\sigma$ with $\phi$:
%     $$
%     MLP(x)\approx\phi(xW_1)(W_2)=(a(xW_1)+b)(W_2)
%     $$
%     Since, the above formula eliminates non-linear transformations, we can now approximate the MLP with the following linear transformation:
%     $$
%     MLP(x)\approx \overline{MLP}(x)=(a(xW_1)+b)(W_2)=xC+B
%     $$
%     where $C\in\mathbb{R}^{d\times d}, B\in\mathbb{R}^{1\times d}$. After the above transformation, the number of parameters in $MLP$ changes from $2\times d\times h$ to $d^{2}+d$ in $\overline{MLP}$. When $h > \frac{d+1}{2}$, the number of parameters becomes smaller. In most of the recent LLMs that adopts the above MLP block (OPT, BLOOM, Falcon, etc.), $h=4d$, which in turn brings a maximun of 87.5\% therotical parameters reduction (when $d\rightarrow\inf$) in MLP blocks.
%     \item MHA: constant foldable with no benefits
% \end{itemize}
% We observe that during neural network inference, part of certain matrix computations remain constant, and can be "pre-computed" aprior to inference.
    
% \begin{figure}
%     \caption{A simple multilayer perceptron (MLP) network with linearly approximated activation function.}
%     \label{fig:mlp-example}
% \end{figure}

% \Cref{fig:mlp-example} shows a simple MLP with an activation function, and how it gets approximated with a linear transformation.
% \begin{itemize}
%     \item MLP without activation: saves xxx\% memory requirement and xxx\% compute.
%     \item Single-head attention: saves xxx\% memory requirement and xxx\% compute.
% \end{itemize}


\subsection{Challenge}
Unfortunately, applying the aforementioned modification to the MLP blocks in a LLM presents a significant challenge: approximating the non-linear activation functions in LLMs with a single linear transformation can incur substantial errors, which severely degrades model performance.
% For non-linear functions in LLMs (e.g., GELU), naively approximating the entire function with a single linear transformation induces severe model performance drop. 

\begin{figure}
    \caption{Input and output distribution of the activation function in Falcon-7B across different MLP layers on the Wikitext-2 dataset.}
    \label{fig:input-output-dist-GELU-falcon}
\end{figure}

To illustrate this, we consider non-linear functions such as the Gaussian Error Linear Unit (GELU)~\cite{hendrycks2023gaussianerrorlinearunits}. A naive approximation of the entire GELU function with a single linear transformation leads to a marked decline in model efficacy.
We investigated the performance impact of naively approximating the activation function with a linear regressor and validated the performance of Falcon-7B on the Wikitext-2 dataset. 
First, we collected the input and output data from the activation function in each layer. Next, we trained a linear regressor to approximate the activation function. Finally, we evaluated the change in perplexity of the model when replacing the activation function in MLP with the linear regressor for each layer.
\Cref{fig:input-output-dist-GELU-falcon}.a shows the distribution of inputs and outputs to the GELU activation function in Falcon-7B on the Wikipedia dataset, which reveals significant discrepancies. We trained a linear regression model based on the collected input-output pairs, depicted as the red line in \Cref{fig:input-output-dist-GELU-falcon}.a. The results indicate that this approximation incurs substantial errors.
We evaluated the model's perplexity with the approximated linear regressor. In our expectations, the model's performance significantly deteriorated. \Cref{fig:input-output-dist-GELU-falcon}.b illustrates that the perplexity increased from \(xxx\) to \(xxx\) on the Wikipedia dataset, indicating a severe degradation in model performance that renders it practically unusable.

To make things worse, substituting the non-linear activation function with a linear one adversely affects the representation capabilities of the MLP within LLMs. According to the universal approximation theorem~\cite{hornik1989multilayer,csaji2001approximation}, non-linear activation functions are essential for learning complex mappings between inputs and outputs. Blindly replacing non-linear functions with linear alternatives restricts the model's ability to learn only linear separable mappings, a limitation that cannot be remedied through subsequent re-training or fine-tuning of the model weights.

% \Cref{fig:input-output-dist-GELU-falcon}.a shows the distribution of the input and output to the GELU activation function in Falcon-7B on Wikipedia dataset. We trained a linear regression model based on the input and output for each layer, which is ploted as the red line in \Cref{fig:input-output-dist-GELU-falcon}.a. We can see from the result that the approximation incures very large errors.
% Next, we evaluated the perplexity of the model with approximated linear regressior. \Cref{fig:input-output-dist-GELU-falcon}.b shows the result, the perplexity increases from xxx to xxx on Wikipedia dataset, which indicates a severe degrate the model performance and makes the model completely unusable.

% To make things worse, changing the non-linear activation function to a linear one could inreversely affect the capability of (the MLPs in) LLM. According to the universal approximation theorem~\cite{hornik1989multilayer,csaji2001approximation}, the non-linear activation function plays a crucial role in learning the complex mapping between input and outputs. Blinding replace the non-linear functions with linear ones makes the model only capable of learning linear separable mappings, and this is inrecoverable through any further re-training or fine-tuning of the model weights.

% \begin{itemize}
%     % \item "Non-linear" operators (e.g., activation function, softmax, layer normalization) breaks "pre-computation chain", resulting in little chance to apply associative and distributive lows to the computation.     
%     \begin{itemize}
%         \item First, approximation introduces extra error, which might hurt model performance. For non-linear functions in LLMs (e.g., GELU), naively approximating the entire function with a single linear transformation induces severe model performance drop. 
%         \begin{figure}
%             \caption{Input and output distribution of the GELU non-linear function in Falcon-7B in different MLP layers on Wikipedia dataset.}
%             \label{fig:input-output-dist-GELU-falcon}
%         \end{figure}
%         We investigated the performance affect introduced by the naive approximation approach.
%         \Cref{fig:input-output-dist-GELU-falcon} shows the distribution of the input and output to the GELU activation function in Falcon-7B on Wikipedia dataset. We trained a linear regression model based on the input and output for each layer, which is ploted as the red line in \Cref{fig:input-output-dist-GELU-falcon}. The perplexity of the model increases from xxx to xxx on Wikipedia dataset, which indicates a severe degrate the model performance.
%         % -> Where these statistics comes from?
%         % -> what the statistics shows?
%         % -> what challenge can be draw?
%         \begin{figure}
%             \caption{Aggregated input distribution of neurals in MLP.}
%             \label{fig:agg-input-distilation}
%         \end{figure}
%         % \item Second, data distribution of the input to non-linear functions changes across different input tokens. Consequently, a static linear approximation strategy can be vunerable to data distribution changes, which limits the generalizability. \Cref{fig:agg-input-distilation} illustrates the input distribution of xxx neurals of the MLP in Falcon-7B. \TODO{re-think the relativness of the evidence}
%     \end{itemize}
%     % \item Certain LLM building blocks increase the number of the parameters in pre-computed matrix.
%     % \begin{itemize}
%     %     \item "Multi head" attention "multiplies" the number of params needed for pre-computation: Introduces 32x the number of params in pre-computing attention heads on LLaMA 2-7B
%     %     \item MLPs involving squared-termd inputs increases the number of parameters when pre-compute: Introduces ~300 $\times$ the number of params in pre-computing "GatedMLP" in LLaMA 2-7B model.
%     % \end{itemize}
% \end{itemize}



==> sections/back_v2.tex <==
\section{Background}
\iffalse
\OUTLINE{
\begin{itemize}
    \item Constant folding with simple example
    \begin{itemize}
        \item What is \cf and its benefits
        \item Example of \cf in a simple program
    \end{itemize}
    \item LLM compression methods: why llm compression is important
    \begin{itemize}
        \item Bottleneck analysis of LLM in inference tasks
        \item How LLM compression levigate the bottleneck
    \end{itemize}
\end{itemize}
}
\fi
%-------------------------------------------------------------------------------
% 用一个paragraph
Constant folding is a compiler optimization technique that evaluates constant expressions at compile time. This optimization leverages the associativity, commutativity, and distributivity of expressions to simplify programs. For instance, the expression \texttt{a=(4*2)+1} can be ``folded'' to \texttt{a=9} at compile time. This technique reduces program code size and runtime computation cost and has been widely adopted in various programming languages, including C/C++~\cite{Optimize87:online}, Python~\cite{TensorFl6:online,pythoncp39:online,ansel2024pytorch}, and SQL~\cite{SparkSQL40:online}.
% In recent years, the emergence of deep learning has seen the adoption of \cf in many deep learning frameworks, such as TensorFlow~\cite{TensorFl6:online}, PyTorch~\cite{pythoncp39:online}, and ONNX~\cite{Graphopt58:online}, improving the efficiency of various DL pipelines~\cite{TensorFl23:online,Develope9:online,TensorRT28:online,TensorFl6:online}.

Recently, large language models (LLMs) have become an active topic in both literature and industry. These models have shown great potential in various natural language processing tasks. However, deploying LLMs for inference tasks is challenging due to their large number of parameters. One of the main reasons is that LLMs work in an auto-regressive manner: the model generates one token at a time, and the output of the previous token is used as the input for the next token. Consequently, each time step requires loading all the model parameters into the cache of the compute unit (e.g., GPU, CPU), leading to high memory bandwidth requirements~\cite{xu2024survey,lin2024awq,wang2024model}.

To address this issue, researchers have proposed various techniques to compress LLMs, including quantization, pruning, knowledge distillation, and low-rank approximation. The key idea of these techniques is to reduce the model size by either reducing the number of parameters or reducing the size of each parameter, which in turn reduces the memory footprint and inference latency of LLMs~\cite{frantar2022optq,lin2024awq,wei2023outlier,kim2023finequant,sun2023simple,ma2023llm,zhang2024plug,gu2023knowledge,timiryasov2023baby,li2023losparse,saha2023matrix,chand2023dsformer}.

% Despite the widespread adoption of \cf in various deep learning workloads optimizations, little research has explored its potential application to LLMs. 
% To understand this gap, we first analyze the key enabler for the application of \cf to DL workloads. Then, we
% compare the workload characteristics of LLMs with deep learning, and shed some light on why LLMs lacks optimization opportunity for \cf.
% - in DL workloads, models structure are more various, for example the 

\section{Opportunity and Challenge}
\iffalse
\OUTLINE{
\begin{itemize}
    \item Opportunity: \cf in LLMs leads to large performance gain
    \begin{itemize}
        \item Basic idea: view activation as a combination of two linear functions, and constant fold the MLP block into a single linear transformation
        \item Illustrating example: \cf in Opt-6.7B with ReLU activation
        \item Evaluation: speedup, memory reduction, and accuracy
    \end{itemize}
    \item Challenge: \cf in LLMs with non-linear activation incurs large error
    \begin{itemize}
        \item Recent trend in LLMs: non-linear activation functions (e.g., GELU, SiLU, ELU, SeLU, GLU) are used to improve model performance
        \item Why direct \cf in LLMs with non-linear activation is not practical
        \item Evaluating the accuracy drop of direct application.
    \end{itemize}
\end{itemize}
}
\fi
Inspired by the success of constant folding in compiler optimizations, we discover a new opportunity to apply constant folding to LLMs to reduce the memory footprint and speedup inference.
% According to the above analysis, the primary barrier preventing LLMs achieving \cf lies in the non-linear transformations that interleave with linear transformations. To enable LLMs to be ``constant foldable'', we must adjust their structural design, allowing multiple linear transformations to chain together seamlessly.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/opportunity_illustration.pdf}
    \caption{Illustration of constant folding in the MLP block of an LLM. The ReLU activation function is approximated by two linear functions, enabling the folding of multiple linear transformations into a single one.}
    \label{fig:mlp_constant_folding_example}
\end{figure}
\subsection{Opportunity}
\label{sec:opportunity}
The key enabler for applying \cf to LLMs is to treat the activation function as linear functions defined on different ranges. Consider OPT as an example, which uses a ReLU activation function in its multilayer perceptron (MLP) module. 
The ReLU activation function can be viewed as a combination of two linear functions: $f(x) = x$ for $x > 0$ and $f(x) = 0$ for $x \leq 0$. As long as the input $x$ is always positive (or negative), the ReLU activation function essentially becomes a linear transformation. 
Under this view, the MLP can be further considered as three linear transformations chained together: $MLP(x)=\phi(xW_1)W_2=a(xW_1)W_2$, where $\phi$ is the ReLU activation function, $a$ is either $0$ or $1$ depending on the input, $W_1\in\mathbb{R}^{d\times h}$ and $W_2\in\mathbb{R}^{h\times d}$ are the weight matrices.
Fortunately, recent studies suggest that more than 90\% of the activation inputs in OPT are negative~\cite{liu2023deja,mirzadehrelu,song2024powerinfer}, leading to a significant opportunity for \cf in the MLP module.
By applying the rules of association, distribution, and commutation for the MLP\footnote{Floting point arithmetics are commutative but not necessarily associative nor distributive due to it's finite range and precision~\cite{SixthCom51:online}.
However, our experiments reveal that the error incured is negeligible in the context of ``folding'' an LLM (\Cref{sec:precision_affects}).}, these linear transformations can be folded into a single one: $MLP(x)=xC$, where $C=aW_1W_2$ and $C\in\mathbb{R}^{d\times d}$. 
After the above transformation, the number of parameters in $MLP$ changes from $2\times d\times h$ to $d^{2}$ in the ``folded'' MLP. When $h > \frac{d+1}{2}$, the number of total parameters of MLP becomes smaller after folding.
In many contemporary LLMs employing this MLP block—such as OPT, BLOOM, and Falcon—\(h\) typically equals \(4d\). This configuration can yield a theoretical parameter reduction of up to 87.5\% in the MLP block, with little impact on the model's accuracy.
\Cref{fig:mlp_constant_folding_example} examplifies the constant folding process in an MLP block with ReLU activation function, where $W_1\in\mathbb{R}^{2\times 4}$ and $W_2\in\mathbb{R}^{4\times 2}$. Consider the case where the input $x$ is always negative (or positive), the total number of parameters in the MLP block is reduced from 16 to 4 after constant folding.

% Consider the case of a MLP. We define a linear transformation function as follows:
\iffalse
Let us consider the case of modifying the non-linear activation function in MLP modules of an LLM. We define a linear transformation $\phi$ as follows:
\[
\phi(x) = ax + b
\]
where \(a, b\) are scaler values. We can approximate the original non-linear function \(\sigma\) in MLP with \(\phi\):
\[
\begin{aligned}
    MLP(x)=\sigma(xW_1)(W_2) \\
    \approx \phi(xW_1)(W_2) = (a(xW_1) + b)(W_2).
\end{aligned}
\]
where $W_1\in\mathbb{R}^{d\times h}$ and $W_2\in\mathbb{R}^{h\times d}$. This formulation effectively eliminates non-linear transformations, enabling us to constant folding the MLP into a simplified linear transformation:
\[
MLP(x) \approx \overline{MLP}(x) = (a(xW_1) + b)(W_2) = xC + B,
\]
where \(C \in \mathbb{R}^{d \times d}\) and \(B \in \mathbb{R}^{1 \times d}\). This transformation significantly alters the weight parameter count in the MLP, reducing it from \(2 \times d \times h\) to \(d^2 + d\) in \(\overline{MLP}\). Notably, when \(h > \frac{d + 1}{2}\), the number of weight parameters decreases after \cf.
In many contemporary LLMs employing this MLP block—such as OPT, BLOOM, and Falcon—\(h\) typically equals \(4d\). This configuration can yield a theoretical parameter reduction of up to 87.5\% (as \(d \rightarrow \infty\)) within the MLP blocks.

Apart from the MLP block, the MHA block can also be modified to increase \cf opportunities. 
However, the benefits of \cf in MHA are minimal, as the resulting folded matrices contains far more parameters than the original matrices. In this paper, we focus on \cf of MLP blocks in LLMs. These blocks takes up 67\%\ to 80\% of the total parameters in LLMs~\cite{almazrouei2023falconseriesopenlanguage,touvron2023llama2openfoundation}, and often takes up much computational and memory resources during inference~\cite{xu2024survey,zhou2024survey,lin2024awq,yuan2024llm}.

% Regarding multi-head attention (MHA), while we can achieve constant folding, the benefits are minimal. 

% The key challenge arises from non-linear operators, which hinder the constant folding process. By addressing these barriers, we can transform LLMs into structures that are amenable to constant folding.
% \begin{itemize}
%     \item To make LLMs constant foldable, an idea would be to modify the internal structure of LLM to increase \cf opportunities.
%     \item The barriers to \cf in LLMs are non-linear operators. If we modify the barriers, LLMs are constant foldable.
%     \item MLP: For example, Let us consider a function that performs linear transformation: $\phi(x)=ax+b$, where $a,b\in\mathbb{R}^{1\times h}$. We approximate the original non-linear function $\sigma$ with $\phi$:
%     $$
%     MLP(x)\approx\phi(xW_1)(W_2)=(a(xW_1)+b)(W_2)
%     $$
%     Since, the above formula eliminates non-linear transformations, we can now approximate the MLP with the following linear transformation:
%     $$
%     MLP(x)\approx \overline{MLP}(x)=(a(xW_1)+b)(W_2)=xC+B
%     $$
%     where $C\in\mathbb{R}^{d\times d}, B\in\mathbb{R}^{1\times d}$. After the above transformation, the number of parameters in $MLP$ changes from $2\times d\times h$ to $d^{2}+d$ in $\overline{MLP}$. When $h > \frac{d+1}{2}$, the number of parameters becomes smaller. In most of the recent LLMs that adopts the above MLP block (OPT, BLOOM, Falcon, etc.), $h=4d$, which in turn brings a maximun of 87.5\% therotical parameters reduction (when $d\rightarrow\inf$) in MLP blocks.
%     \item MHA: constant foldable with no benefits
% \end{itemize}
% We observe that during neural network inference, part of certain matrix computations remain constant, and can be "pre-computed" aprior to inference.
    
% \begin{figure}
%     \caption{A simple multilayer perceptron (MLP) network with linearly approximated activation function.}
%     \label{fig:mlp-example}
% \end{figure}

% \Cref{fig:mlp-example} shows a simple MLP with an activation function, and how it gets approximated with a linear transformation.
% \begin{itemize}
%     \item MLP without activation: saves xxx\% memory requirement and xxx\% compute.
%     \item Single-head attention: saves xxx\% memory requirement and xxx\% compute.
% \end{itemize}
\fi
\begin{figure}
    \centering
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figure/pdfs/falcon7b/c4/layer_10_neural_kde.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figure/pdfs/falcon7b/c4/layer_30_neural_kde.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figure/pdfs/falcon7b/wikitext2/layer_10_neural_kde.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figure/pdfs/falcon7b/wikitext2/layer_30_neural_kde.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figure/pdfs/falcon7b/ptb/layer_10_neural_kde.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figure/pdfs/falcon7b/ptb/layer_30_neural_kde.pdf}
    \end{subfigure}
    \caption{Density estimation of the activation function input distribution for 100 neurals of layer 10 and 30 in Falcon-7B. Each curve represents the kernel density estimation of the input distribution for a single neural. The upper two figures is for C4, 
    the middle two figures are for Wikitext-2,
    and the lower two figures are for PTB.}
    \label{fig:neural-act-inputs}
\end{figure}
\subsection{Challenge}
Despite the potential benefits of \cf in LLMs, recent trends in LLMs have shifted towards using more complicated non-linear activation functions, including 
GELU~\cite{hendrycks2016gaussian}, SiLU~\cite{elfwing2018sigmoid}, ELU~\cite{clevert2015fast}, SeLU~\cite{klambauer2017self}, and GLU~\cite{dauphin2017language}, for better convergence and final accuracy~\cite{almazrouei2023falconseriesopenlanguage,shazeer2020gluvariantsimprovetransformer}.
For example, models like GPT-2/3, BLOOM, and Falcon use GELU activation function; and models like LLaMA, Qwen use SiLU. 
To understand the recent trend of activation functions used in the most popular open-source LLMs, we manually analyzed the type of activation function used in the top 15 text generation models (LLMs) on HuggingFace~\cite{Transf37:online}, one of the most popular model repositories, and found that 7 use GELU, 8 use SiLU, and non of them use ReLU activation function.

These activation function are smoother but more complicated than ReLU, making direct application of \cf to the MLP module impractical.
% Unfortunately, applying the aforementioned modification to the MLP blocks in a LLM presents a significant challenge: approximating the non-linear activation functions in LLMs with a single linear transformation can incur substantial errors, which severely degrades model performance.
% For non-linear functions in LLMs (e.g., GELU), naively approximating the entire function with a single linear transformation induces severe model performance drop. 
% \begin{figure}
%     \caption{Input and output distribution of the activation function in Falcon-7B across different MLP layers on the Wikitext-2 dataset.}
%     \label{fig:input-output-dist-GELU-falcon}
% \end{figure}
To illustrate this, we consider the GELU activation function.
Naively regarding GELU as two linear transformation ($f(x) = x$ for $x > 0$ and $f(x) = 0$ for $x \leq 0$, see \Cref{sec:opportunity}) can lead to a marked decline in model efficacy.
% Naive approximation of the entire GELU function with a single linear transformation leads to a marked decline in model efficacy.
We investigated the performance impact of the naive approximation approach by replacing the GELU activation function with two linear regressors, one for $x \leq 0$ and the other for $x > 0$, in the MLP module of Falcon-7B and validated the performance of the model on the Wikitext-2 dataset~\cite{merity2016pointer}. 
Specifically, we collected the input and output data from the activation function in each layer. Next, we trained the linear regressors with the collected data to approximate the activation function for each layer.
% \Cref{fig:input-output-dist-GELU-falcon}.a shows the distribution of inputs and outputs to the GELU activation function in Falcon-7B on the Wikitext-2 dataset, revealing significant discrepancies. 
% The red line in \Cref{fig:input-output-dist-GELU-falcon}.a represents the linear regressors trained on the collected input-output pairs.
We evaluated the model's perplexity with these linear regressors. As expected, the model's performance significantly deteriorated: the perplexity (lower the better) increased from \(6.59\) to \(750.3\) on the Wikitext-2 dataset, indicating a severe degradation in model performance that renders it practically unusable.

% Moreover, substituting the non-linear activation function with a linear one adversely affects the representation capabilities of the MLP within LLMs. Non-linear activation functions are essential for learning complex mappings between inputs and outputs~\cite{hornik1989multilayer,csaji2001approximation}. Blindly replacing non-linear functions with linear alternatives restricts the model's ability to learn only linearly separable mappings, a limitation that cannot be remedied through subsequent re-training or fine-tuning of the model weights.

% \Cref{fig:input-output-dist-GELU-falcon}.a shows the distribution of the input and output to the GELU activation function in Falcon-7B on Wikipedia dataset. We trained a linear regression model based on the input and output for each layer, which is ploted as the red line in \Cref{fig:input-output-dist-GELU-falcon}.a. We can see from the result that the approximation incures very large errors.
% Next, we evaluated the perplexity of the model with approximated linear regressior. \Cref{fig:input-output-dist-GELU-falcon}.b shows the result, the perplexity increases from xxx to xxx on Wikipedia dataset, which indicates a severe degrate the model performance and makes the model completely unusable.

% To make things worse, changing the non-linear activation function to a linear one could inreversely affect the capability of (the MLPs in) LLM. According to the universal approximation theorem~\cite{hornik1989multilayer,csaji2001approximation}, the non-linear activation function plays a crucial role in learning the complex mapping between input and outputs. Blinding replace the non-linear functions with linear ones makes the model only capable of learning linear separable mappings, and this is inrecoverable through any further re-training or fine-tuning of the model weights.

% \begin{itemize}
%     % \item "Non-linear" operators (e.g., activation function, softmax, layer normalization) breaks "pre-computation chain", resulting in little chance to apply associative and distributive lows to the computation.     
%     \begin{itemize}
%         \item First, approximation introduces extra error, which might hurt model performance. For non-linear functions in LLMs (e.g., GELU), naively approximating the entire function with a single linear transformation induces severe model performance drop. 
%         \begin{figure}
%             \caption{Input and output distribution of the GELU non-linear function in Falcon-7B in different MLP layers on Wikipedia dataset.}
%             \label{fig:input-output-dist-GELU-falcon}
%         \end{figure}
%         We investigated the performance affect introduced by the naive approximation approach.
%         \Cref{fig:input-output-dist-GELU-falcon} shows the distribution of the input and output to the GELU activation function in Falcon-7B on Wikipedia dataset. We trained a linear regression model based on the input and output for each layer, which is ploted as the red line in \Cref{fig:input-output-dist-GELU-falcon}. The perplexity of the model increases from xxx to xxx on Wikipedia dataset, which indicates a severe degrate the model performance.
%         % -> Where these statistics comes from?
%         % -> what the statistics shows?
%         % -> what challenge can be draw?
%         \begin{figure}
%             \caption{Aggregated input distribution of neurals in MLP.}
%             \label{fig:agg-input-distilation}
%         \end{figure}
%         % \item Second, data distribution of the input to non-linear functions changes across different input tokens. Consequently, a static linear approximation strategy can be vunerable to data distribution changes, which limits the generalizability. \Cref{fig:agg-input-distilation} illustrates the input distribution of xxx neurals of the MLP in Falcon-7B. \TODO{re-think the relativness of the evidence}
%     \end{itemize}
%     % \item Certain LLM building blocks increase the number of the parameters in pre-computed matrix.
%     % \begin{itemize}
%     %     \item "Multi head" attention "multiplies" the number of params needed for pre-computation: Introduces 32x the number of params in pre-computing attention heads on LLaMA 2-7B
%     %     \item MLPs involving squared-termd inputs increases the number of parameters when pre-compute: Introduces ~300 $\times$ the number of params in pre-computing "GatedMLP" in LLaMA 2-7B model.
%     % \end{itemize}
% \end{itemize}



==> sections/intro.tex <==
\section{Introduction}
Constant folding is a compiler optimization techinque used by many modern compilers. 
Recent years, \cf has been adopted in many deep learning frameworks (e.g.,TensorFlow~\cite{TensorFl6:online}, PyTorch~\cite{pythoncp39:online} and ONNX~\cite{Graphopt58:online}) to optimize the computation graph in deep learning workloads.
Constant folding identifies and evaluates constant expressions at compile time rather than at runtime. The benefits of \cf include reducing runtime computational cost and reducing source code size.

Despite the benefits, \cf has not been adopted in the recent bloom of large language model (LLM) workloads. Different from deep learning (DL) workloads, LLM workloads have unique characteristics that deep learning workloads does not have.
First, LLMs usually have similiar model architectures, but models in deep learning workloads usually employs different architectures for different tasks.
Mainstream LLMs (e.g., GPT~\cite{openai2024gpt4technicalreport,brown2020languagemodelsfewshotlearners}, LLaMA~\cite{touvron2023llamaopenefficientfoundation,touvron2023llama2openfoundation,grattafiori2024llama3herdmodels} and Falcon~\cite{almazrouei2023falconseriesopenlanguage}, etc.) are based on the transformer architecture~\cite{vaswani2023attentionneed}. The transformer architecture consists of multiple layers of self-attention and feed-forward neural networks. 
The self-attention layer is usually followed by a feed-forward neural network layer. 
% The FFNN layer usually consists of two linear transformations separated by an activation function (e.g., ReLU). The activation function is usually followed by a layer normalization layer.
One key advantage of LLMs is that they are general-purpose models. The enormous number of weight parameters allows a single LLM to be used in wide ranges of applications, such as text generation, translation, and summarization. On the countary, deep learning models are usually tailored to specific tasks, and different tasks usually need different models. For example, a model for image classification (e.g., ResNet~\cite{he2015deepresiduallearningimage}, VGG~\cite{simonyan2015deepconvolutionalnetworkslargescale}) usually shares different architecture from a model for object detection (e.g., YOLO~\cite{redmon2016lookonceunifiedrealtime}, RetinaNet~\cite{lin2018focallossdenseobject}). Similiarly, in natural language processing, various models with different architecture (e.g., Seq2seq~\cite{sutskever2014sequence}, LSTM~\cite{hochreiter1997long}, RNN~\cite{medsker2001recurrent}, BERT~\cite{devlin2019bertpretrainingdeepbidirectional}) are designed for different tasks\GS{TODO: check whether the claim is correct}, such as text classification, named entity recognition, and question answering.

Second, LLM workloads require less data preprocessing efforts than deep learning workloads. 
Specifically, LLMs are directly interfaced with natural languages, whereas DL models usually need data preprocessing to convert the raw data into a format that the model can understand. For example, a DL model for text classification~\cite{BART83:online} needs to first clean the input test to remove special characters, and then convert the raw text into a numerical representation (e.g., word embedding) before feeding it into the model. 
Additionally, it needs to pre-define the number of classes and the class labels for the model. 
Interacing with LLMs is more straightforward: the model can directly take the tokenized text as input and generate the output in the same format, without data preprocessing efforts. 
In summary, in terms of model architecture and data preprocessing, LLM workloads are generally simpler than deep learning workloads. This simplier nature of LLM workloads makes it harder to apply \cf, as \cf requires a certain level of complexity in the model architecture and data preprocessing pipeline to be effective.

% Finally, the runtime performance bottleneck of LLM workloads is different from deep learning workloads. 

% This unique characteristic of LLMs makes it difficult to apply \cf to LLM workloads.
% LLM workloads have unique characteristics that make \cf not applicable. 

This paper present \sys, a new approach that increases the \cf opportunity for LLM, and reduce the computational cost and memory footprint for LLM inference accordingly. The idea of \sys is to approximate the non-linear activation function in LLMs with linear ones to increase the \cf opportunity. However, the direct approximation of the activation function in LLMs with linear functions is not practical, as the linear approximation incurs significantly large error. 
To address this issue, \sys only approximate the activation function with linear functions for a part of the ``hot'' input ranges, guided by the observation that the distribution of activation input in LLMs are skewed. Consequently, \sys performs \cf for the neurals with activation inputs falling into ``hot'' input ranges. 
For neurals with activation inputs outside of the approximated ranges, \sys leverages an online predictor to identify them, and falls back to the original activation function computation for the neurals.
% For ``cold'' input ranges that are not approximated, \sys falls back to the original activation function computation.

Although the idea behind \cf is simple, \sys can supressingly reduce the memory footprint by up to 70\% with a relative small model performance drop. This result even surpasses some state-of-the-art LLM pruning methods.
% Our experiments show that \sys can reduce the memory footprint by a up to 70\% relative small model performance drop. This result supasses the state-of-the-art LLM pruning methods.

The contributions of this paper are as follows:\GS{TODO: add this}
% \begin{itemize}
%     \item 
% \end{itemize}
% \begin{itemize}
%     \item What is constant folding? 
%     \begin{itemize}
%         \item Overall: Constant folding is a compiler optimization techinque used by many modern compilers, including TensorFlow and PyTorch that optimize deep learning workflows.
%         \item What constant folding does: identify and evaluate constant expressions at compile time rather than at runtime.
%     \end{itemize}
%     \item The benefits of constant folding:
%     \begin{itemize}
%         \item Reduce runtime computational cost. \GS{TODO: add example}
%         \item Reduce source code size. \GS{TODO: add example}
%     \end{itemize}
%     \item Despite the benefits, constant folding has not been  adopted in the recent bloom of large language model (LLM) workloads.
%     \begin{itemize}
%         \item Workload characteristics of LLM:
%         \item Reason why constant folding not applipable to LLM workloads:
%     \end{itemize}
%     \item We presents \sys, a new approach that increases the constant folding opportunity for LLM, and reduce the computational and memory footprint for LLM inference accordingly.
%     \item Though the idea behand constant folding is simple, our experiments show that \sys can reduce the memory footprint by a xxx, and speedup inference by xxx with relative small model performance drop.
%     \item Contributions: \GS{TODO}
% \end{itemize}

==> sections/intro_cf_and_prune.tex <==
% \section{Introduction}
% \label{sec:intro}

% 1. 在大模型场景下，模型size大，不要写edge device；2. inference时间长
% meanwhile constant folding is a compiler optimization technique that reduces the program code size and runtime computation cost.
% this paper tries to answer the question: can we apply constant folding to large language models to reduce the memory footprint during inference
% acc, size, inference time

% -----------------------

% CF
% Opporty in LLM
% Challenges
Deploying large language models on edge devices is beneficial  in several perspectives, such as reducing latency, enhancing privacy, and enabling offline inference to reduce cost of cloud services.
However, deploying large language models on edge devices is challenging due to their large memory requirements. 
To address this issue, researchers have proposed various techniques to compress large language models, such as quantization, pruning, knowledge distillation, and low-rank approximation. 
The idea of these techniques is to reduce the model size via either reducing the number of parameters or reducing the size of each parameter.

meanwhile, constant folding is a compiler optimization technique that reduces the program code size and runtime computation cost.xxx
Similiar to reducing the model size, constant folding is a compiler optimization technique that reduces the program code size and runtime computation cost. 
It has been widely adopted in machine learning frameworks, such as TensorFlow~\cite{TensorFl6:online}, PyTorch~\cite{pythoncp39:online}, and ONNX~\cite{Graphopt58:online}, to optimize the computation graph of machine learning models.
Despite the wide adoption of constant folding in machine learning frameworks, we found that constant folding has limited performance improvement by analyzing 161 deep learning and large language models: the average inference speedup is only 1.03$\times$.

Fortunately, we observed that constant folding can be very useful in large language models.
We presents \sys, a novel approach that enhances constant folding opportunities in large language models to reduce the memory footprint during inference. 
The key idea of \sys is to approximate the non-linear activation function in large language models with linear ones to increase the constant folding opportunity.
However, the direct approximation of the activation function in large language models with linear functions is not practical, as the linear approximation incurs significantly large error.
To address this issue, \sys only approximates the activation function with linear functions for a part of the "hot" input ranges, guided by the observation that the distribution of activation input in large language models are skewed.
Consequently, \sys performs constant folding for the neurons with activation inputs falling into "hot" input ranges.
For neurons with activation inputs outside of the approximated ranges, \sys leverages an online predictor to identify them and falls back to the original activation function computation for the neurons.

Although the idea behind constant folding is simple, \sys can surprisingly reduce the memory footprint by up to 70\% without fine-tuning. Compared with recent structural and unstructural pruning methods, \sys achieves xxx lower perplexity under the same compression ratio. better than all existing pruning/unstructural methods.

% \begin{itemize}
%     \item importance of LLM compression
%     \begin{itemize}
%         \item Why need llm compression: Deploying large language models on edge devices is beneficial for many applications, such as speech recognition, language translation, and text generation.
%         \item challenging due to their large memory footprint
%         \item llm compression reduces memory footprint and inference latency: such as quant, pruning, knowledge distillation, lora,etc.
%         \item the key idea is to reduce the model size via either reducing the number of parameters or reducing the size of each parameters.
%     \end{itemize}
%     \item Akin to reducing the model size, constant folding is a compiler optimization that precomputes constant expressions to reduce code size and runtime computation.
%     \item importance of constant folding in compiler optimization (traditional pl, dl frameworks)
%     \item we study xxx models and find that constant folding is not that useful in optimizing xxx models since xxx.
%     \item We show that: constant folding can be very useful in llm by approximating activation function with linear ones.
%     \item experiments show that our approach can reduce the memory footprint by up to 70\% with minimal performance degradation, outperforming recent structural and unstructural pruning methods. In addition, our approach is orthogonal to existing compression techniques, and we can combine them to further reduce the memory footprint.
% \end{itemize}

==> sections/intro_cf_and_prune_v2.tex <==
\section{Introduction}
\label{sec:intro}

% 1. 在大模型场景下，模型size大，不要写edge device；2. inference时间长
% meanwhile constant folding is a compiler optimization technique that reduces the program code size and runtime computation cost.
% this paper tries to answer the question: can we apply constant folding to large language models to reduce the memory footprint during inference
% acc, size, inference time

Recently, transformer-based large language models (LLMs) have revolutionized natural language processing, demonstrating remarkable capabilities across diverse tasks. However, deploying these models for inference is challenging due to their enormous number of parameters, often reaching billions or even trillions~\cite{googlesw98:online}.
Various techniques have been proposed to compress LLMs, including pruning~\cite{sun2023simple,ma2023llm,zhang2024plug}, quantization~\cite{frantar2022optq,lin2024awq,yao2022zeroquant}, knowledge distillation~\cite{gu2023knowledge,timiryasov2023baby}, and low-rank approximation~\cite{li2023losparse,saha2023matrix,chand2023dsformer}.
While pruning has gained popularity due to its simplicity~\cite{yangllmcbench}, it often leads to significant accuracy degradation under high compression ratios - a 80\% compression could result in up to 70\% accuracy loss.

Drawing inspiration from the success of \cf~\cite{Constant13:online} in traditional compiler optimizations, we approach this challenge from a novel perspective: leveraging \cf to compress LLMs while maintaining better accuracy under aggressive compression ratios.
Constant folding, a well-established compiler optimization technique that reduces program code size and runtime computation costs, has been widely adopted in various programming languages including C/C++~\cite{Optimize87:online}, Python~\cite{pythoncp39:online}, and SQL~\cite{SparkSQL40:online} for decades.
We identify a unique opportunity to apply \cf to LLMs for model compression.
Taking the OPT~\cite{zhang2022opt} model family as an example, we can apply \cf to its feed-forward network (FFN) block. 
The key idea is to view the activation function in FFN as linear functions.
Specifically, the FFN in OPT model consists of two matrix multiplications separated by a ReLU activation function.
\textit{By treating the activation function as a combination of two linear functions defined on different ranges}, we can apply the associative property to the two matrix multiplications in FFN, simplifying them into a single multiplication with a smaller matrix.
This transformation achieves up to 87.5\% (\Cref{sec:opportunity}) reduction in FFN parameters for LLMs.

However, a recent trend in LLMs is to use variants of ReLU activation that are faster to converge and improves final accuracy, such as GELU~\cite{hendrycks2016gaussian} and SiLU~\cite{elfwing2018sigmoid}. 
For example, GPT-3~\cite{brown2020language}, one of the most popular LLMs, uses GELU activation function; and BLOOM~\cite{le2023bloom}, a more recent LLM with up to 176B parameters, uses a improved variant of GELU activation function.
These non-linear activation functions are smoother but more complicated than ReLU, which prevents direct application of constant folding to the FFN block.

In this paper, we present \sys, a novel approach that enables constant folding in LLMs with non-linear activation functions such as GELU and SiLU.
Our key insight is that the inputs to these activation functions in LLMs are typically concentrated within a narrow range during inference.
This distribution pattern allows us to \textit{partially} approximate the non-linear activation function with a linear function in the "hot" input ranges (where most values occur), introducing minimal approximation error.
For outlier inputs that fall outside these ranges, \sys employs an efficient online predictor to identify them and dynamically falls back to the original activation function computation.
Extensive experiments demonstrate that \sys reduces the FFN weight matrices by up to 80\%, while significantly outperforming state-of-the-art pruning methods in accuracy. Compared to leading pruning methods like Wanda and RIA, \sys achieves up to 62\% higher accuracy on downstream tasks. For inference, \sys delivers up to 1.6× end-to-end speedup on the state-of-the-art vLLM serving system~\cite{10.1145/3600006.3613165}, and 1.4× speedup on HuggingFace's widely-used implementation~\cite{Transf37:online}.
%  - achieving \textbf{111}$\times$ and \textbf{581.3}$\times$ better perplexity, and \textbf{2.23}$\times$ and \textbf{2.17}$\times$ higher accuracy on average.
% In terms of the tradeoff between inference speedup and performance degradation, \sys outperforming all state-of-the-art structural and unstructural pruning methods.
% In addition, our approach is orthogonal to existing compression techniques, and we can combine them to further improve the efficiency of LLMs.

The key contributions of this paper are:
\begin{itemize}
    \item We identify a novel opportunity to apply constant folding to LLMs. Our method treats activation functions as partially linear functions, reducing FFN block parameters by up to 87.5\%.
    \item We introduce \sys, a new system for constant folding in modern LLMs. It handles non-linear activation functions through partial linear approximation and includes efficient fallback mechanisms.
    \item We conduct extensive experiments with \sys. Results show up to 80\% parameter reduction. This significantly outperforms current state-of-the-art pruning approaches.
\end{itemize}

\iffalse
\begin{itemize}
    \item Importance of LLM: llm have attracted significant attention in recent years with their ability to solve various tasks in natural language processing, such as text generation, translation, and summarization.
    \item However, the cost of deploying large language models for inference tasks is high due to their large memory requirement.
    \item Existing works on llm compression reduces memory footprint and inference latency: such as quant, pruning, knowledge distillation, lora,etc.
    \item the key idea is to reduce the model size via either reducing the number of parameters or reducing the size of each parameters.

    \item Meanwhile, constant folding is a compiler optimization that precomputes constant expressions to reduce code size and runtime computation.
    \item importance of constant folding in compiler optimization (traditional pl, including dl frameworks)
    \item We observed that constant folding can be applied to LLMs with great potential.
    \begin{itemize}
        \item the ReLU activation function is basically combination of two linear functions: 
        \item linear function in MLP can offer great constant folding opportunity. 
    \end{itemize}
    \item However, due to the xxx and xxx reason, GELU and SiLU activation functions are widely used in most recent LLMs. On HuggingFace, xxx of xxx models use ReLU, all other models use xxx which are non-linear and cannot apply constant folding directly.
    
    \item We presents \sys, a novel approach that enables constant folding in LLMs with GELU activation function. The key insight is that the GELU activation function can be approximated by a linear function in the "hot" input ranges, where most inputs occur.
    \item experiments show that our approach can reduce the memory footprint by up to 70\% with minimal performance degradation, outperforming recent structural and unstructural pruning methods. In addition, our approach is orthogonal to existing compression techniques, and we can combine them to further reduce the memory footprint.
\end{itemize}
\fi

==> sections/non_linear_approx.tex <==
\subsection{Non-linear Function Approximation}
\subsubsection{Problem Formulation}
\label{sec:non_linear_approx}
\sys approximates part of the non-linear activation function in FFNs with linear function. Formally, given a FFN with two fully connected layers $FC_1$ and $FC_2$, two weight matrices $W_1\in\mathbb{R}^{d\times h}$ and $W_2\in\mathbb{R}^{h\times d}$, and an input $\textbf{x}\in\mathbb{R}^{k\times d}$ from the calibration dataset ($k$ is the number of tokens), the FFN\footnote{To ease presentation, we omit the bias part.} is defined as:
$$
\begin{aligned}
FC_{1}(\textbf{x})=\sigma(\textbf{x}W_{1}),\ 
FC_{2}(\textbf{x})=FC_{1}(\textbf{x})W_{2}\\
FFN(\textbf{x})=FC_{2}(FC_1(\textbf{x}))
\end{aligned}
$$
where $\sigma$ is the activation function.
The weight matrices can be viewed as a concatation of multiple neurons~\cite{liu2023deja,song2024powerinfer}, each of which has a weight vector $W_{1_{:,n}}\in\mathbb{R}^{d\times 1}$ (one column) and $W_{2_{n,:}}\in\mathbb{R}^{1\times d}$ (one row) in $W_1$ and $W_2$, respectively. The FFN has a total of $h$ neurals.
Our goal is to approximate the activation function $\sigma$ with linear functions for each neuron in the FFN within specific ``hot'' input ranges:
$\phi_n(\textbf{x}W_{1_{:,n}})\approx \sigma(\textbf{x}W_{1_{:,n}})$
where $\phi_n$ is the approximated linear function for neural $n$, $\sigma$ is the original activation function. After the approximation, the FFN can be simplified into a single weight matrix $C\in\mathbb{R}^{d\times d}$ and a bias vector $B\in\mathbb{R}^{1\times d}$: 
\begin{equation}
FFN(\textbf{x})\approx\sum_{n}^{h} \phi_n(\textbf{x}W_{1_{:,n}})W_{2_{n,:}}=\textbf{x}C+B
\label{eq:folded_mlp}
\end{equation}

\subsubsection{Tradeoffs between Accuracy and Matrix Storage}
There exists a fundamental tradeoff between approximation accuracy and storage requirements in our linear approximation approach.
While using more linear ranges for approximation yields higher accuracy—as shorter ranges enable better local linear approximations of non-linear functions—it leads to an exponential increase in the storage overhead of the constant-folded matrices.

This exponential growth occurs because according to \Cref{eq:folded_mlp}, the folded matrix $C$ and bias vector $B$ are derived from the combined linear approximation parameters (slopes and intercepts) of \textit{all} neurons. When any neuron uses multiple linear ranges, it necessitates distinct $C$ and $B$ matrices for each possible combination of range selections across neurons. Formally, with $R$ linear ranges per neuron and $h$ neurons in a layer, the total number of required matrix pairs $(C, B)$ becomes $R^h$. Given that typical large language models have FFNs with $h>10,000$ neurons, storing multiple ranges per neuron quickly becomes computationally intractable.
\Cref{fig:too_many_matrices} demonstrates this exponential growth problem with a simplified example where each neuron uses two linear ranges, resulting in four distinct set of folded weight matrices ($C_{1}\sim C_{4}$, $B_1\sim B_4$).
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/too_many_matrices.pdf}
    \caption{Example of the exponential growth in the number of folded matrices.}
    \label{fig:too_many_matrices}
\end{figure}

\subsubsection{Single Range Approximation Strategy}
To address the exponential storage challenge, \sys employs a constrained approach where each neuron is approximated using exactly one linear range. This strategy utilizes a greedy search algorithm to identify optimal approximation ranges that maximize input coverage while maintaining accuracy.
Formally, for each neuron $n$, we find a linear function $y=ax+b$ that approximates the activation function within a specific input range $[l_1, l_2)$. The approximation function $\phi_n$ is defined as:
$$
\phi_{n}(\textbf{x})=\left\{
\begin{aligned}
a\textbf{x}+b & , & l_1\le x < l_2 \\
\sigma(\textbf{x}) & , & otherwise 
\end{aligned}
\right.
$$

The approximation error for the entire FFN is defined as the sum of individual neuron errors:
$$
err(\textbf{x})=\sum_{n}^{h}err_{n}(\textbf{x})
$$
where the error for each neuron is computed using the L2 norm:
$$
err_{n}(\textbf{x})=||\sigma(\textbf{x}W_{1_{:,n}})W_{2_{n,:}}-\phi_n(\textbf{x}W_{1_{:,n}})W_{2_{n,:}}||_2
$$
\noindent
\textbf{Adaptive Thresholding.}
We next decide how much (threshold) input should fall into the linear range for each neural in each layer.
Given the non-uniform importance of layers and neurons (\Cref{sec:insight}), we adopt an adaptive thresholding mechanism.
For each layer $i$ and neuron $n$, we assign thresholds $t_i$ and $t_{i_n}$ respectively, determined by solving two optimization problems:

For layer-level thresholds:
$$
\begin{aligned}
minimize\sum_{i}^{L}E_{i}t_{i},\ 
s.t.,\sum_{i}^{L}t_{{i}}=tL
\end{aligned}
$$

For neuron-level thresholds:
$$
\begin{aligned}
minimize\sum_{n}^{N}E_{i_n}t_{i_n},\ 
s.t.,\sum_{n}^{N}t_{i_n}=t_{i}N
\end{aligned}
$$
where $E_i$ represents the total empirical error of layer $i$ and $E_{i_n}$ represents the error contribution of neuron $n$ in layer $i$, both measured on a calibration dataset. The first constraint ensures the average threshold across all $L$ layers equals the target threshold $t$, while the second constraint ensures the average threshold across all $N$ neurons in layer $i$ equals that layer's threshold $t_i$.
\input{algo/linear_range_generation.tex}

\noindent
\textbf{Range Searching.}
For each neuron, \sys employs an efficient greedy search strategy to determine the optimal linear approximation range, following these steps. 
1) Initialize a starting range centered at the input distribution's centroid, computed using kernel density estimation (KDE)~\cite{terrell1992variable,parzen1962estimation}. 
2) Gradually expand the range boundaries until reaching the neuron-specific coverage threshold $t_{i_n}$.
3) During expansion, select the direction (left or right) that produces minimal approximation error.
4) Once the optimal range is determined, fit a linear function using least squares regression.
The complete algorithm is formalized in \Cref{alg:linear_range_generation}, leveraging a small calibration data to ensure both approximation accuracy and computational efficiency without fine-tuning the model.

==> tables/portion-input-stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llll}
    \hline
    Dataset & \multicolumn{1}{c}{Falcon-7B} & \multicolumn{1}{c}{Bloomz-7B1} & \multicolumn{1}{c}{GPT2-XL} \\ \hline
    C4                            &                          &  &  \\
    \multicolumn{1}{r}{Wikitext2} & \multicolumn{1}{r}{0.82} & \multicolumn{1}{r}{0.82} &  \\
    PDB                           &                          &  &  \\ \hline
    \end{tabular}%
    }
    \caption{Percentage of input that falls into the linearly approximated ranges when threshold set to 0.85 for LLMPrumer}
    \label{tab:portion-input-stats}
    \end{table}

==> tables/ppl-wikitext2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
  \centering
  \resizebox{0.8\textwidth}{!}{%
  \begin{tabular}{@{}llllllllll@{}}
  \toprule
  Metohd/Model           & \multicolumn{3}{c}{Falcon-7B}              & \multicolumn{3}{c}{Bloomz-7B1}                & \multicolumn{3}{c}{GPT2-XL}                   \\ \midrule
  Dense            & \multicolumn{3}{c}{6.59}                   & \multicolumn{3}{c}{14.12}                     & \multicolumn{3}{c}{17.41}                     \\
  \textit{Sparisty} &
    \multicolumn{1}{c}{\textit{30\%}} &
    \multicolumn{1}{c}{\textit{50\%}} &
    \multicolumn{1}{c}{\textit{70\%}} &
    \multicolumn{1}{c}{\textit{30\%}} &
    \multicolumn{1}{c}{\textit{50\%}} &
    \multicolumn{1}{c}{\textit{70\%}} &
    \multicolumn{1}{c}{\textit{30\%}} &
    \multicolumn{1}{c}{\textit{50\%}} &
    \multicolumn{1}{c}{\textit{70\%}} \\
  Wanda            & 6.8          & 8.4          & 65.0         & 14.6          & 16.6          & 41.1          & 17.7          & 19.8          & 175.1         \\
  RIA              & \textbf{6.7} & 7.3          & 23.2         & 14.4          & 15.9          & 34.7          & \textbf{17.6} & 19.4          & 107.8         \\
  LLMFolder (Ours) & \textbf{6.7} & \textbf{6.9} & \textbf{7.3} & \textbf{13.9} & \textbf{14.9} & \textbf{16.2} & 17.8          & \textbf{19.3} & \textbf{39.9} \\ \bottomrule
  \end{tabular}%
  }
  \caption{Perplexity of different models on Wikitext-2 dataset, when compressed with different methods. Text in \textbf{bold} indicates the best result.}
  \label{tab:ppl-wikitext2}
  \end{table*}

==> tables/zero_shot_falcon.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
    \centering
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{@{}llllllllll@{}}
    \toprule
    Metohd           & \multicolumn{3}{c}{PIQA}                      & \multicolumn{3}{c}{Lambada}                   & \multicolumn{3}{c}{ARC-Challenge}             \\ \midrule
    Dense            & \multicolumn{3}{c}{79.5\%}                    & \multicolumn{3}{c}{74.5\%}                    & \multicolumn{3}{c}{40.3}                      \\
    \textit{Sparisty} &
      \multicolumn{1}{c}{\textit{30\%}} &
      \multicolumn{1}{c}{\textit{50\%}} &
      \multicolumn{1}{c}{\textit{70\%}} &
      \multicolumn{1}{c}{\textit{30\%}} &
      \multicolumn{1}{c}{\textit{50\%}} &
      \multicolumn{1}{c}{\textit{70\%}} &
      \multicolumn{1}{c}{\textit{30\%}} &
      \multicolumn{1}{c}{\textit{50\%}} &
      \multicolumn{1}{c}{\textit{70\%}} \\
    Wanda            & 79.5          & 78.1          & 63.3          & \textbf{77.0} & 78.4          & 35.3          & 39.7          & 35.5          & 20.6          \\
    RIA              & \textbf{79.8} & 78.6          & 70.3          & 75.0          & \textbf{73.8} & 46.5          & 39.1          & 37.8          & 26.4          \\
    LLMPruner (Ours) & 79.6          & \textbf{79.1} & \textbf{78.4} & 74.1          & 73.0          & \textbf{74.3} & \textbf{40.5} & \textbf{38.9} & \textbf{35.7} \\ \bottomrule
    \end{tabular}%
    }
    \caption{Falcon 7B zero-shot accuracy (\%) of downstream tasks.}
    \label{tab:zero-shot-falcon}
    \end{table*}
